SiTe CiM: Signed Ternary Computing-in-Memory for Ultra-Low Precision Deep Neural Networks

Ternary Deep Neural Networks (DNN) have shown a large potential for highly energy-constrained systems by virtue of their low power operation (due to ultra-low precision) with only a mild degradation in accuracy. To enable an energy-efficient hardware substrate for such systems, we propose a compute-enabled memory design, referred to as SiTe-CiM, which features computing-in-memory (CiM) of dot products between signed ternary (SiTe) inputs and weights. SiTe CiM is based on cross-coupling of two bit cells to enable CiM of dot products in the signed ternary regime. We explore SiTe CiM with 8T-SRAM, 3T-embedded DRAM (3T-eDRAM) and 3T-ferroelectric metal FET (FEMFET) memories. We propose two flavors of this technique, namely SiTe CiM I/II. In SiTe CiM I, we employ two additional transistors per cell for cross-coupling, achieving fast CiM operations, albeit incurring an area overhead ranging from 18% to 34% (compared to standard ternary memories). In SiTe CiM II, four extra transistors are utilized for every 16 cells in a column, thereby incurring only 6% area cost (but leading to slower CiM than SiTe CiM I). Based on the array analysis, our designs achieve up to 88% lower CiM latency and 78% CiM energy savings across various technologies considered, as compared to their respective near-memory computing counterparts. Further, we perform system level analysis by incorporating SiTe CiM I/II arrays in a ternary DNN accelerator and show up to 7X throughput boost and up to 2.5X energy reduction compared to the near-memory ternary DNN accelerators.

==> Sections/Array.tex <==
\section{Array Design with SiTe CiM I/II}
\label{sec:array}

\begin{figure}[t!]
\centering
  \includegraphics[width = 0.98\linewidth]{Figures/Figure 7.PNG}
  \caption{Array architecture of SiTe CiM I/II cells.}
  \label{fig:array}
  %\vspace{-2.5mm}
\end{figure}

We begin with a broad description of SiTe CiM I/II arrays. In a SiTe CiM I based array, $WWL$, $RWL_1$ and $RWL_2$ connect cells in a row together. $BL$, $BLB$ (in 8T-SRAM), $WBL_1$, $WBL_2$ (in 3T-eDRAM/3T-FEMFET), and $RBL_1$ and RBL2 are shared along the column in SiTe CiM I as well as SiTe CiM II based arrays (Fig. ~\ref{fig:array}). In addition, in SiTe CiM II, $LRBL_1$ and $LRBL_2$ are shared along the column by the cells of a block (Fig. ~\ref{fig:site2}(a)) and $WWL$, $RWL$, $RWL_{t1}$, $RWL_{t2}$ are laid out along the row  (Fig. ~\ref{fig:array}). 

Next, we elaborate the architecture of SiTe CiM I/II array to highlight its capability to perform massively parallel vector-matrix multiplication operations. Recall, we establish that 8 word line assertions are ideal for restricting errors within bounds during MAC computations (Section ~\ref{sec:design}). In addition to the sensing failures (Section ~\ref{sec:design}), the maximum number of simultaneously accessed cells in a column is determined by another factor – sparsity. While a large ternary output aggravates error, their occurrence probability is low since $>$ 40\% vector elements in DNNs are zeroes due to sparsity \cite{tim_dnn,sparse_tnn}. Considering both
factors, the work in \cite{tim_dnn} shows that $N_V$ =16 rows can be simultaneously asserted while limiting the maximum output of 8 and approximating all outputs $>$ 8 to be equal to 8.  This approximation leads to a probability of error $<$ 1.5e-4 and has been shown to have no impact on DNN accuracy in \cite{tim_dnn}. We follow the same method as \cite{tim_dnn} to assert 16 rows in one cycle while  utilizing a 3-bit Flash ADC to determine the final dot-product ($\leq$ 8).

To further improve parallelism, we design our arrays to consist of 16 blocks ($N_{B}$), wherein each block is designed with $N_C$ = 256 columns and $N_R$ =16 rows (Fig. ~\ref{fig:array}).
Hence, each block has the capability of executing $N_{MAC}$ = $N_C$ = 256 MAC operations simultaneously, with vector size $N_V$ =16. Next, partial outputs (sums) from each block is stored in peripheral compute unit (PCU) using a sample and hold circuitry and are accumulated after multiple block accesses to result in the
final dot products. We utilize the TiM DNN architecture \cite{tim_dnn} to design our macros with 32 PCUs ($<$ $N_C$=256) for the entire array, to limit the overheads due to peripherals \cite{tim_dnn}. Finally, the dot products are quantized, and passed through an activation function to obtain the inputs to the next DNN layer.

==> Sections/DesignOrig.tex <==
\section{Design of Signed Ternary (SiTe) Computation-in-Memory (CiM) Cells Utilizing Cross-Coupling of Bit Cells}
\label{sec:designorig}

\begin{figure}[t!]
\centering
  \includegraphics[width = 0.95\linewidth]{Figures/Figure 2.PNG}
  \caption{(a) Schematic of SiTe CiM I cell. Inset shows that the underlying cell/storage element can be 8T-SRAM, 3T-eDRAM or 3T-FEMFET cell, (b) symbol of a SiTe CiM I cell.}
  \label{fig:site_cells}
  %\vspace{-2.5mm}
\end{figure}

In this section, we propose two cells capable of signed ternary computation in memory namely SiTe CiM I and SiTe
CiM II. We use the technique of cross-coupling two bitcells by adding extra access transistors to them for achieving CiM of dot product in the signed ternary regime i.e. $inputs \in [-1, 0, 1]$ and $weights \in [-1, 0, 1]$. Although we present their analysis with 8T-SRAM, 3T-eDRAM and 3T-FEMFET cells in this work, the proposed method can be utilized for bit cells of other memory technologies, especially those with separated read-write paths. We incur an overhead of two read transistors per cell for SiTe CiM I (Fig. ~\ref{fig:site_cells}(a)). However, this overhead can be reduced to four transistors per sixteen cells in SiTe CiM II (Fig. 5(a)), albeit at the cost of compute performance. Compared to previous implementations of the ternary cells \cite{tim_dnn}, our proposed designs incur minimal area cost, as discussed subsequently.

\renewcommand\thesubsectiondis{\arabic{subsection}.} 
\renewcommand\thesubsubsectiondis{\alph{subsubsection}.}
\renewcommand\theparagraphdis{\arabic{paragraph}.}

\subsection{SiTe CiM I Cell}

SiTe CiM I cell consists of two memory bit cells ($M_1$, $M_2$) at its core (Fig. ~\ref{fig:site_cells}). In this work, $M_1$ and $M_2$ correspond to 8T-SRAMs, 3T-eDRAMs or 3T-FEMFETs (Fig. ~\ref{fig:site_cells}(a) and inset). $M_1$ and $M_2$ store binary bit information ‘0’ (high resistance state (HRS)) or ‘1’ (low resistance state (LRS)) either in the form of (a) charge (SRAM/eDRAM), or (b) polarization (FEMFET). Combination of stored weights in $M_1$/$M_2$ constitute a ternary weight ($W$) (Fig. 3(a)), for which we employ differential encoding. For $W$ = 0, both $M_1$ and $M_2$ = 0 (HRS). For $W$ = 1(-1), $M_1$ = 1(0) and $M_2$ = 0(1). SiTe CiM I cell (Fig. ~\ref{fig:site_cells}) features a write wordline ($WWL$) associated with write access transistor(s) and bit lines (e.g., $BL_{1,2}$/$BLB_{1,2}$ in 8T-SRAM, $BL_1$/$BL_2$ in 3T-eDRAM and 3T-FEMFET) for programming $M_1$ and $M_2$. Each of $M_1$ and $M_2$ possess read access transistors, $AX_1$ and $AX_2$ connected to read bit lines $RBL_1$ and $RBL_2$, respectively and controlled with the read word line ($RWL_1$). Further, we add access transistors, $AX_3$ and $AX_4$ and a second read wordline ($RWL_2$) in SiTe CiM I to cross-couple $M_1$ and $M_2$ for signed ternary CiM (Fig. ~\ref{fig:site_cells}(a)). Notice that $AX_3$ connects $M_1$ to $RBL_2$ while $AX_4$ connects $M_2$ to $RBL_1$ in a cross-coupled fashion when $RWL_2$ is asserted. Only $RWL_1$ is asserted for read, while $RWL_1$ or $RWL_2$ are asserted for compute in accordance with ternary input ($I$) encoding (Fig. 3(b)). Like $W$, differential encoding is used for $I$. When $I$ is 0, both $RWL_1$ and $RWL_2$ are 0. When $I$ is 1(-1), $RWL_1$ is driven to $V_{DD}$ (0) and $RWL_2$ is driven to 0 ($V_{DD}$). Interaction of ternary weight ($W$) and input ($I$) produces ternary scalar product ($O$), that is encoded based on combination of $RBL_1$ and $RBL_2$ voltages (Fig. 3(c) - discussed later). For voltage-based sensing, when both $RBL_1$ and $RBL_2$ remain precharged at $V_{DD}$, $O$ is 0. When $RBL_1$ discharges to $V_{DD} - \Delta V$ and $RBL_2$  remains at $V_{DD}$, $O$ is 1. Similarly, when $RBL_2$ discharges to $V_{DD} - \Delta V$ and $RBL_1$  remains at $V_{DD}$, $O$ is -1. In a similar way, we can use current-based sensing, in which current through RBLs encodes the scalar product. For SiTe-CiM 1, we employ voltage-sensing due to its higher energy efficiency compared to current-sensing.   

Next, we discuss write, read, and CiM of scalar products and dot products in SiTe CiM I.

\begin{figure}[t!]
\centering
  \includegraphics[width = 0.98\linewidth]{Figures/Figure 3.PNG}
  \caption{(a) Weight, (b) input, (c) output encoding, (d) truth table for ternary scalar product computation, (e-f) examples of scalar multiplication in SiTe CiM.}
  \label{fig:site_encoding}
  %\vspace{-2.5mm}
\end{figure}

\subsubsection{Write and Read Operations in SiTe CiM I}

\paragraph{Write}
Writing into a SiTe CiM I cell is equivalent to writing into the two binary memory elements, $M_1$ and $M_2$ (as described in Section ~\ref{sec:background}). Based on the ternary value ($W)$ to be written into the cell, $M_1$ and $M_2$ can be programmed according to the encoding in Fig. 3(a). 

\paragraph{Read}
Read is performed by first pre-charging $RBL_1$ and $RBL_2$ to $V_{DD}$ and asserting $RWL_1$ to $V_{DD}$. When sensing $W$ = 1 (-1) , $RBL_2$ ($RBL_1$) remains at $V_{DD}$ while $RBL_1$ ($RBL_2$) drops to $V_{DD} - \Delta V$ (Fig. 3(c)). For $W$ = 0, both $RBL1$ and $RBL2$ remain at $V_{DD}$. Note that doring read, $BL$/$BLB$ in 8T-SRAM are kept in a pre-charged state ($V_{DD}$)  whereas for 3T-eDRAM/FEMFET, $WBL$ is kept at 0V. It should be noted that $RWL_2$, which enables the cross-coupling between $M_1$ and $M_2$, is kept off during read and is only used for the signed ternary CiM operation. Thus, the read operation is equivalent to performing conventional reads on $M_1$ and $M_2$ in parallel. 

\subsubsection{Scalar Product Computation in SiTe CiM I}
Ternary scalar product ($O = I*W$) is obtained as a combined outcome of $RBL_1$ and $RBL_2$ voltages (Fig. ~\ref{fig:site_encoding}(c-d)) in response to different ternary weight ($W$) and input ($I$) combinations. To initiate the scalar product computation, both $RBL_1$ and $RBL_2$ are precharged to $V_{DD}$. Next, $RWL_1$ and $RWL_2$ are asserted based on the input value (Fig. ~\ref{fig:site_encoding}(b)). Let us consider different cases on-by-one below:

\paragraph{$I$ = 1}
For this input, $RWL_1 = V_{DD}$, $RWL_2 =$ 0 and $O = I*W = W$. Thus, the scalar product in this case is identical to reading out the weight value. For $W$ = 0, both $RBL1$ and $RBL2$ remain at $V_{DD}$, hence $O$ = 0 (Fig. ~\ref{fig:site_encoding}(c)). When $W$ = 1 (-1), $O$ = 1 (-1) since $RBL_1$ ($RBL_2$) has a low resistance path to ground through $AX_1$ ($AX_2$), discharging it to $V_{DD} - \Delta V$, whereas $RBL_2$ ($RBL_1$) stays at $V_{DD}$. An example illustrating this case is given in Fig. ~\ref{fig:site_encoding} (e). 

\paragraph{$I$ = -1}
For this input, $RWL_1$ = 0, $RWL_2 = V_{DD}$ and $O = I*W = -W$. Thus, the scalar product in this case is \textit{negative} of the weight value. By asserting $RWL_2$, the cross-coupled transistors $AX_3$ and $AX_4$ are turned on. Consequently, it is the cross-coupling that enables the change of sign of the sensed weight value. When $W$ = 1 (i.e. $M_1=1$ and $M_2=0$), $O$ = -1. This is because $RBL_2$ has a low resistance path to ground through $AX_3$ and $M_1$, discharging it to $V_{DD} - \Delta V$. On the other hand, $RBL_1$ stays at $V_{DD}$ as it is connected to the $M_2$ via $AX_4$ (Fig. ~\ref{fig:site_encoding}(c)). Similarly, when $W$ = -1 (i.e. $M_1=0$ and $M_2=1$), the opposite happens (i.e. $RBL_1$ discharges while $RBL_2$ stays at $V_{DD}$ due to cross-coupling), producing $O=1$. When $W$ = 0, both $RBL_1$ and $RBL_2$ remain at $V_{DD}$ leading to $O$ = 0. An example illustrating this case is given in Fig. ~\ref{fig:site_encoding} (f).  

\paragraph{$I$ = 0}
For this input, both $RWL_1$ and $RWL_2$ = 0, and $O = I*W = 0$. Since both read wordlines are off, all the read access transistors ($AX_{1,2,3,4}$) are in off state. Thus, both $RBL_1$ and $RBL_2$ remain at their precharged voltage value of $V_{DD}$. 

\subsubsection{Signed Ternary MAC Operation using SiTe CiM I}
To accomplish signed ternary MAC computation, we assert multiple rows of the memory array simultaneously in accordance with their respective input values.  We then sense the $RBL_1$ and $RBL_2$ voltages resulting from the collective action of the proposed ternary cells corresponding to the accessed rows. Recall that $RBL_1$ discharging by $\Delta V$ corresponds to the scalar product output of 1 while $RBL_2$ discharging by $\Delta V$ indicates -1 respectively. Hence, if '\textit{N}' rows are activated simultaneously, out of which ‘\textit{a}’ scalar multiplications produce an output of 1 and ‘\textit{b}’ scalar multiplications produce an output of -1, then the final $RBL_1$ and $RBL_2$ voltages are $V_{DD} - a\Delta V$ and $V_{DD} - b\Delta V$ respectively \cite{tim_dnn}. Similar to \cite{tim_dnn}, We employ 3-bit flash analog to digital converters (ADCs) on each RBL to yield digital values corresponding to ‘\textit{a}’ and ‘\textit{b}’. (The reasons for choosing 3-bit ADC is discussed subsequently.) The final dot product is given by $\sum_{i=1}^{N} I_{i}*W_{i}$ = a-b, which is achieved by subtracting ‘b’ from ‘a’ using a 3-bit digital CMOS subtractor. Fig. ~\ref{fig:site_variation}(a) illustrates this operation. 

\subsubsection{Sense Margin and Variation Analysis of Signed Ternary MAC using SiTe CiM I}
An important question pertaining to the effectiveness of signed ternary MAC operations with SiTe CiM I is the maximum number of rows that can be accessed during one MAC computation. To analyze this, we study $RBL$ voltage discharge characteristics as a function of the output on the $RBL$s ($a$ or $b$) and extract the sense margin (SM) (= half the difference of RBL voltages between two adjacent output values). When the expected $RBL$ output increases from 1 to 8, SM reduces from 50mV to 40mV and becomes even lower for higher values. We attribute this to the exponential behavior of bit-line capacitance discharging. The decreasing SM limits the number of cells that can be simultaneously asserted. However, note that inherent sparsity of DNNs also plays a role in relaxing this limitation (as discussed in Section ~\ref{sec:array}). 

Further, we study the effect of threshold voltage ($V_{TH}$) variation on SM. We report our observation based on analysis of FEMFET based SiTe CiM I. Since the read/compute path is similar for 8T-SRAM and 3T-eDRAM based SiTe CiM I, we observe similar trends for them. We consider a standard deviation of 6$\sigma$ = 120mV for $V_{TH}$ for all the transistors in FEMFET SiTe CiM I \cite{variation}. We perform
1000 Monte-Carlo SPICE simulations, shown in Fig. ~\ref{fig:site_variation}(d) for cases corresponding to $RBL$ outputs of 1 to 8. As the output increases, greater overlap of $RBL$ voltage between adjacent states is observed. This implies a heightened probability of sensing error with an increase in the output values (Fig. ~\ref{fig:site_variation}(e)). 

Although the above factors related to device/array variation characteristics impart cautionary conclusions for outputs larger than 8, sparsity in DNNs (detailed discussion in Section IV) could help alleviate this constraint. Specifically, sparsity in DNNs (presence of significant weights/inputs as zero values) lowers probability of occurrence of large output values. This is especially true for ternary precision DNNs, which contain a high percentage of zero weights/inputs \cite{sparse_tnn}. This directly affects the probability of error in the dot-product which is equal to the product of sensing error probability (calculated based on Monte Carlo simulations) and the occurrence probability of a particular output value. Fig. ~\ref{fig:site_variation}(d) shows a non-monotonic trend in the dot product error probability plotted as a function of output values. Finally, we calculate the total probability of error ($P_e$) during the dot product operation as the sum of errors observed for each output (Fig. ~\ref{fig:site_variation}(e)), which amounts to 3.10e-3. In other words, for every 1000 MAC operations we have $\sim$3 errors with magnitude $\pm$1 (since only adjacent states overlap, as seen in Fig. ~\ref{fig:site_variation}(e)). The system-level evaluations in \cite{tim_dnn} reveal that a $P_e$ of 3.10e-3 (corresponding to outputs of up to 8) has negligible impact on accuracy of DNNs, attributed to the low magnitude of errors and resiliency of DNNs to computational errors.


\begin{figure}[t!]
\centering
  \includegraphics[width = 0.98\linewidth]{Figures/Figure 4.PNG}
  \caption{Column of SiTe CiM I cells showing ternary dot-product computation using input ($I$) and weight ($W$) vector, (b) an example of worst-case input-weight combination for maximum $RBL$ discharge, (c) $RBL$ voltage vs number of no. of discharges, (d) probability of MAC error with increasing discharges, (e) variation in $RBL$ discharge summarized from 1000 Monte Carlo samples for each discharge state.}
  \label{fig:site_variation}
  %\vspace{-2.5mm}
\end{figure}

\begin{figure*}[t!]
\centering
  \includegraphics[width = 0.97\textwidth]{Figures/Figure 5.PNG}
  \captionsetup{justification=centering}
  \caption{(a) Schematic of a column of SiTe CiM II cells, (b) weight, (c) input, (d) output encoding, (e) truth table for ternary scalar product computation, (f-g) examples of scalar multiplication in SiTe CiM II, (h) dot product computation in a column of SiTe CiM II cells.}
  \label{fig:site2}
  %\vspace{-2.5mm}
\end{figure*}

\subsection{SiTe CiM II Cell}
Let us now present the second flavor of the SiTe CiM design (referred to as SiTe CiM II), which aims to mitigate the area overheads of SiTe CiM I. Instead of employing two cross-coupled transistors ($AX_3$ and $AX_4$) per ternary cell (as in SiTe CiM I), the SiTe CiM II design utilizes four additional transistors for every \textit{16} cells of a column  to facilitate ternary CiM by means of cross-coupling  (Fig. ~\ref{fig:site2}(a)). Based on this arrangement, we define a block to comprise 16 (rows) x 256 (columns). An array is then formed with 16 blocks or 256 (rows) x 256 (columns).  Due to the sharing of the cross-coupling transistors amongst 16 cells,  we achieve significant area benefits over SiTe CiM I, which is quantified in Section ~\ref{sec:system}. 

In SiTe CiM II (Fig. ~\ref{fig:site2}(a)), the storage elements ($M_1$ and $M_2$) and write mechanisms (using $BL$s and $WWL$) are similar to SiTe CiM I (Fig. 2(a)). The difference between SiTe CiM I and SiTe CiM II is in the design of their read/compute paths. Notice that in SiTe CiM II, read access transistors $AX_1$ and $AX_2$ associated with $M_1$ and $M_2$ connect to local read bit lines, $LRBL_1$ and $LRBL_2$ respectively (Fig. ~\ref{fig:site2}(a)). $LRBL_1$ and $LRBL_2$ are shared by the 16 cells along the column of a block. In contrast, $RBL_1$ and $RBL_2$ are shared by all (256) cells in the column of an array. $AX_1$ and $AX_2$ are activated by $RWL$ that runs along the row (256 cells). In addition, four other access transistors $AX_{t1M1}$, $AX_{t1M2}$, $AX_{t2M1}$ and $AX_{t2M2}$ (marked as shared transistors in Fig. ~\ref{fig:site2}(a)) are used in SiTe CiM II. $AX_{t1M1}$ and $AX_{t1M2}$ are accessible through read wordline $RWL_{t1}$. They connect $LRBL_{1}$ and $LRBL_{2}$ to $RBL_1$ and $RBL_2$ respectively. $AX_{t2M1}$ connects $LRBL_1$ to $RBL_2$ and $AX_{t2M2}$ connects $LRBL_2$ to $RBL_1$ using read wordline $RWL_{t2}$. $RWL_{t1}$ and $RWL_{t2}$ are shared along a row. The inclusion of $AX_{t2M1/M2}$ along with $RWL_{t2}$ allows us to encode signed ternary $I$ = -1 which, in turn, realizes cross-coupling of $M_1$ to $RBL_2$ and $M_2$ to $RBL_1$ for signed ternary output (details discussed later). It is important to note that current-based sensing is used in this design instead of voltage-based sensing (which was employed for SiTe CiM I). This is because voltage-sensing may lead to incorrect sensing of binary value ‘0’ caused by charge sharing between $LRBL$ and $RBL$. The said issue further aggravates when multiple rows are activated to accomplish CiM. Current-based sensing helps in circumventing this concern. In other words, while SiTe CiM II poses a restriction for the sensing to be current-based,  SiTe CiM I cells are compatible with both voltage and current-based sensing. Next, we explain write-read operations.


\subsubsection{Write and Read Operations in SiTe CiM II}
\paragraph{Write}
 Similar procedure as SiTe CiM I (discussed previously) is followed to store $W$ in SiTe CiM II cells (Fig. ~\ref{fig:site2}(b)).

\paragraph{Read}
In order to read, $RBL_1$ and $RBL_2$ are driven to $V_{DD}$. Then, $RWL_i$ and $RWL_{t1}$ are asserted while $RWL_{t2}$ is kept at 0V (subscript $i$ denotes the $i^{th}$ row in the block being read). The said biasing creates a path for current to flow from $RBL_1$ ($RBL_2$) via $AX_1$ ($AX_2$) and $AX_{t1M1}$ ($AX_{t1M2}$) when $M_1$($M_2$) stores 1. The current is sensed on $RBL_1$ and $RBL_2$ to determine the stored ternary weight ($W$). For ternary '0' ($M_1$ = 0 and $M_2$ = 0), $I_{HRS}$ is sensed on both $RBL_1$ and $RBL_2$. Note that $I_{HRS}$ here mainly results from a small current that flows from $RBL_2$ to charge the capacitor of $LRBL_2$. Negligible current flows through $M_1$/$M_2$ when either is in HRS.  When sensing ternary ‘1’ ($M_1$ = 1 and $M_2$ = 0), we obtain $I_{LRS}$ and $I_{HRS}$ on $RBL_1$ and $RBL_2$ respectively (similar to Fig. ~\ref{fig:site2}(f)).  For ternary ‘-1’ ($M_1$ = 0 and $M_2$ = 1), currents available on $RBL_1$ and $RBL_2$ are $I_{HRS}$ and $I_{LRS}$, respectively. 

\subsubsection{Obtaining Scalar Product in SiTe CiM II}
As mentioned earlier, weights are encoded as a combination of bits stored in $M_1$ and $M_2$ like in SiTe CiM I (Fig. ~\ref{fig:site2}(b)). The inputs are encoded as a combination of $RWL$, $RWL_{t1}$ and $RWL_{t2}$ as shown in Fig. ~\ref{fig:site2}(c). The ternary scalar product outputs depend on currents appearing on $RBL_1$/$RBL_2$ ($I_{RBL1}$/$I_{RBL2}$) and is equal to their subtracted value (Fig. ~\ref{fig:site2}(d)). We detail this with examples below: 

\paragraph{$I$ = 1}
For this input, $RWL$ = $V_{DD}$, $RWL_{t1}$ = $V_{DD}$, $RWL_{t2}$ = 0 and $O = I*W = W$. This case is similar to the read operation. Hence, for $W$ = 1 ($M_1$ = 1/LRS and $M_2$ = 0/HRS), we receive $I_{RBL1}$ = $I_{LRS}$ and $I_{RBL2}$ = $I_{HRS}$. As described above, we perform subtraction of the RBL currents to obtain $O$ = $I_{LRS}$ – $I_{HRS}$ = 1 (Fig. ~\ref{fig:site2}(f)). When $W$ = -1 ($M_1$ = 0/HRS and $M_2$ = 1/LRS), $I_{RBL1}$ = $I_{HRS}$ and $I_{RBL2}$ = $I_{LRS}$; $O$ = $I_{HRS}$ – $I_{LRS}$ = -1. For $W$ = 0, $I_{RBL1}$ = $I_{RBL2}$ = $I_{HRS}$, $O$ = 0.

\paragraph{$I$ = -1}
For this input, $RWL$ = $V_{DD}$, $RWL_{t1}$ = 0, $RWL_{t2}$ = $V_{DD}$ and $O = I*W = -W$. Turning on $RWL_{t2}$ enables the cross-coupling between $M_1$ and $M_2$. For $W$ = 1 ($M_1$ = 1, $M_2$ = 0), we achieve $I_{RBL1}$ = $I_{HRS}$ and $I_{RBL2}$ = $I_{LRS}$. Hence, $O$ = $I_{HRS}$ – $I_{LRS}$ = -1 (Fig. ~\ref{fig:site2}(g)). Conversely, when $W$ = -1, $I_{RBL1}$ = $I_{LRS}$, $I_{RBL2}$ = $I_{HRS}$ and $O$ = $I_{LRS}$ – $I_{HRS}$ = 1. In case of $W$ = 0, $O$ = $I_{HRS}$ – $I_{HRS}$ = 0.

\paragraph{I = 0}
For this input, $RWL$ = $RWL_{t1}$ = $RWL_{t2}$ = 0 and $O = I*W = 0$. Since all read word lines are at 0V, all read access transistors are off, preventing current flow through $RBL_1$ and $RBL_2$. Hence, $O$ = 0.

\subsubsection{Signed Ternary MAC Operation using SiTe CiM II}
Like in SiTe CiM I, multiple rows are accessed for computing ternary MAC output. However, multi-row access  in SiTe CiM II is attainable only when each accessed row belongs to \textit{distinct} blocks. We illustrate this in Fig. ~\ref{fig:site2}(h) wherein the accessed row of each block (without any loss of generality) is shown with inputs marked. Recall that read access transistors $AX_{t1M1/M2}$ and $AX_{t2M1/M2}$ in SiTe CiM II are shared within the block, hence a common $RWL_{t1}$/$RWL_{t2}$ is associated with the 16 column cells in a block (Fig. ~\ref{fig:site2}(h)). Thus, for the cells within the same block, distinct values of the input vector must be applied in different cycles. In other words,  one row from each block is asserted in a given cycle to compute MAC output. Hence, it takes \textit{N} cycles for the entire computation. (where \textit{N} is the number of cells in a block).   

It is noteworthy that even in SiTe CiM I, despite the option to simultaneously apply distinct inputs on all the rows, only 16 rows were accessed in a single cycle. This was done to maintain sufficient sense margins and counter variation-induced errors, thus sacrificing parallelism to some extent for compute robustness. SiTe CiM II takes into account this robustness-driven constraint to group multiple cells in a block and share the cross-coupling transistors amongst those cells. The choice of the size of the block is dictated by the targets for the amount of parallelism, CiM latency (determined in part by the interaction of the LBLs and BLs) and the layout footprint.     

After multiple rows are asserted, currents due to the interaction of $I_i$ and $W_i$ in each row aggregate on $RBL_1$ and $RBL_2$. $I_{RBL1}$ and $I_{RBL2}$ are then used to evaluate the dot-product as follows. First, a comparator is used to determine which of $I_{RBL1}$ and $I_{RBL2}$ has higher current and its output represents the sign of the MAC output ($S$). If $I_{RBL1} > I_{RBL2}$, $S$ = 1, otherwise $S$ = -1. Then the comparator output along with $I_{RBL1}$ and $I_{RBL2}$ is fed to a current subtractor circuit which determines the magnitude
of the difference of $I_{RBL1}$ and $I_{RBL2}$. $|I_{RBL1}-I_{RBL2}|$ is an integral
multiple ‘n’ of $I_{LRS}$ - $I_{HRS}$. We extract the value of ‘n’ by utilizing an ADC (more information in Section ~\ref{sec:array}). We provide an example here to illustrate our MAC
computation using SiTe CiM II. Let $I_{RBL1}$ = a$I_{LRS}$+ (16 - a)$I_{HRS}$, $I_{RBL2}$ = c$I_{LRS}$ + (16 - c)$I_{HRS}$ and $I_{RBL2} > I_{RBL1}$. This indicates that the comparator output is $S$ = -1 as per our previous discussion. Then,  we employ the subtractor to get $I_{RBL2}$ - $I_{RBL1}$ = (c-a)($I_{LRS}$ - $I_{HRS}$). When this is passed to the ADC, we obtain n = c-a. The final MAC output is $O$ = $S$*n = a-c.

\subsubsection{Sense Margin (SM) and Variation Analysis of Signed Ternary MAC using SiTe CiM II}

\begin{figure}[t!]
\centering
  \includegraphics[width = 0.98\linewidth]{Figures/Figure 6.PNG}
  \caption{Examples of dot product output = 1 using inputs and weights for (a) maximum loading effect and (b) minimum loading effect, (c) sense margin for expected output 0 through 16.}
  \label{fig:site2_variation}
  %\vspace{-2.5mm}
\end{figure}

Here, we study SM as a function of MAC outputs using SiTe CiM II cells. We perform this analysis to establish the maximum number of simultaneous row assertions for MAC operation similar to the exercise done for the SiTe CiM I cell. We present our approach of analyzing sense margin for SiTe CiM II using the examples shown in Fig. ~\ref{fig:site2_variation}(a-b). In both cases, we expect $O$ = 1, however the weight and input combinations applied in the two cases are different. In Fig. ~\ref{fig:site2_variation}(a), which we refer to as example (a), we use ($I_1$, $W_1$) = (1,1) whose outcome is $I_{RBL1}$ = $I_{LRS}$ and $I_{RBL2}$ = $I_{HRS}$. For the remaining rows, i.e., row 2-16, we set ($I_{2..16}$, $W_{2..16}$) = (1,0). Corresponding to $W$ = 0 and $I$ = 1 for these rows, we obtain non-zero currents on $RBL_1$ and $RBL_2$ due to their interaction with $L_{RBL1}$ and $L_{RBL2}$, respectively, i.e., $I_{RBL1}$ =15$I_{HRS}$ and $I_{RBL2}$ =15$I_{HRS}$ (Fig. ~\ref{fig:site2}(e)). Combining total current on $RBL_1$ and $RBL_2$ from all the rows, we have $I_{RBL1}$ = $I_{LRS}$ +15$I_{HRS}$ and $I_{RBL2}$ = 16$I_{HRS}$¸ and finally $O$ = $I_{RBL1}$ - $I_{RBL2}$ = $I_{LRS}$ - $I_{HRS}$ = 1.

In Fig. ~\ref{fig:site2_variation}(b), which we refer to as example (b),  we start with ($I_1$, $W_1$) = (1,1), i.e., $I_{RBL1}$ = $I_{LRS}$ and $I_{RBL2}$ =$I_{HRS}$. However, for rows 2-16, our inputs and weights are ($I_{2..16}$, $W_{2..16}$) = (0,0). Since, $I_{2..16}$ = 0, no current contribution on $RBL_1$ and $RBL_2$ is observed from those rows. Overall, we observe $I_{RBL1}$ = $I_{LRS}$ and $I_{RBL2}$ = $I_{HRS}$¸ and $O$ = $I_{RBL1}$ = $I_{LRS}$ - $I_{HRS}$ = 1. 

Notice that for identical outputs in examples (a) and (b), $I_{RBL1/2,a} > I_{RBL1/2,b}$, where $I_{RBL1/2,a}$ and $I_{RBL1/2,b}$ are the read bit line currents for example (a) and (b), respectively. For $O$ = 1, example (a) is the worst case (WC) example leading to the maximum current in the $RBL$s since rows with $W$ = 0 also contribute to $RBL$ current. This results in the largest loading of the sensing circuitry, leading to largest deviation of the output current from the ideal current (i.e. with sensing resistance = 0). Whereas example (b) is the best case (BC) i.e. least loading, since only the row with $W$ = 1 is solely responsible for $RBL$ current resulting in the minimum current. We perform a similar exercise to identify BC/WC examples for all outputs $\leq$ 16 and ultimately obtain the respective $I_{RBL1/2}$ values. Finally, for an expected output $O_{(n-1) \leftrightarrow n}$, we define SM margin as ($O_{BC,n}$ - $O_{WC,n-1}$)/2. Fig. ~\ref{fig:site2_variation}(c) shows SM calculated using this method. We observe from Fig. ~\ref{fig:site2_variation}(c), that the SM begins to diminish for $O$ $>$ 8. This is similar to our prior observation during the analysis of the SiTe CiM I cell, where the SM reduced to indistinguishable levels once $O$ $>$ 8. Thus, SM analysis provides us with a consistent parameter for parallel assertion of rows in both SiTe CiM I and II cells to be used for their array design. That being said, the sparsity present in DNN weights/inputs will also play an important part in determining the degree of parallel row assertion, as discussed in detail in the upcoming section.  
